Transformer visualization via dictionary learning: contextualized embedding as a linear superposition of transformer factors

Transformer networks have revolutionized NLP representation learning since they were introduced. Though a great effort has been made to explain the representation in transformers, it is widely recognized that our understanding is not sufficient. One important reason is that there lack enough visualization tools for detailed analysis. In this paper, we propose to use dictionary learning to open up these "black boxes" as linear superpositions of transformer factors. Through visualization, we demonstrate the hierarchical semantic structures captured by the transformer factors, e.g., word-level polysemy disambiguation, sentence-level pattern formation, and long-range dependency. While some of these patterns confirm the conventional prior linguistic knowledge, the rest are relatively unexpected, which may provide new insights. We hope this visualization tool can bring further knowledge and a better understanding of how transformer networks work. The code is available at https://github.com/zeyuyun1/TransformerVis

==> html_file.tex <==
dim: 170 \\ 2nd street tunnel and part of downtown los angeles spread
out over a 48@-@ hour period. kesha explained the idea behind the video
as well as the experience during an interview with mtv news; she said
that the video was different from her other videos, noting that it was
going to show a sexier side of herself. the music video for" we r who we
r" is presented as an underground party. the video starts off with
futuristic flashing lights. kesha, seen in a ponytail wearing gray and
black makeup, chains, ripped stockings, and a sparkly one@-@ piece
leotard made of shards of broken\\\\ and several european territories),
her" endless love" duet with luther vandross( number@-@ one in new
zealand) and" against all odds" featuring westlife( number@-@ one in the
united kingdom)." thank god i found you" was also omitted from the
japanese track listing, and replaced with" all i want for christmas is
you". for the album artwork, carey launched a social media campaign on
april 12, 2015, whereby fans had to share a link to her website in order
to reveal the cover which was concealed by a curtain. using the
hashtag``\textless{} unk\textgreater{}'',\\\\ single," we belong
together". he contained to add" but still, if mimi ' s going to mine
from her own extensive back catalog of ballads, those are the primo
melodies to go for." a reviewer for dj booth thought that minaj" ruined"
the song.=== music video=== the accompanying music video for the remix
of" up out my f ace" was directed by carey' s husband, nick cannon.
minaj spoke about filming a video with carey and how she did not believe
that the video would ever be released:" i didn ' t even tell anyone i
shot a video with\\\\ the producer, few days after he had finished the
composition, madonna completed writing the lyrics of" i don' t give a".
solveig understood that the lyrics were probable references towards
madonna' s life and thus received coverage in the press. however, he was
not aware of the inner meaning behind the lyrics. with billboard
magazine, the producer further explained: at first i thought we were
going to work on one song; that was the original plan. let' s try to
work on one song and take it from there-- not spend too much time
thinking about the l egend, and do something that just makes sense.\\\\
provided an additional and assistant engineering. all the instruments
were provided by eriksen and hermansen while dean sang the background
vocals. in may 2011, in the mix review, an analyzing commercial
productions, mike senior of sound on sound revisited the original mixing
of the song. according to him, before he started the mix, senior played
the song a couple of times before releasing what thing about it" bugged"
him. working it out, he noted that the harmony of the mix is undermined
by the kick drum." what' s my name?" contains basic harmonies that are a
bar of f minor, a bar of a major\\\\ practiced in their backyards and
at\textless{} unk\textgreater{} salon, owned by knowles' s mother, tina.
the group would test routines in the salon, when it was on montrose
boulevard in houston, and sometimes would collect tips from the
customers. their try out would be critiqued by the people inside. during
their school days, girl' s tyme performed at local gigs. when summer
came, mathew knowles established a" boot camp" to train them in dance
and vocal lessons. after rigorous training, they began performing as
opening acts for established r\& b groups of that time such as swv, dru
hill and immature. tina\\\\ day reception at the greek embassy. upon
return to greece, she was greeted at the airport by fans along with the
music video of" my number one" playing on the video monitors. while in
greece, she attended the opening ceremony of the european final four for
the volleyball champions league in\textless{} unk\textgreater{}, where
her song was played as she appeared on stage with cheerleaders. on march
29, paparizou arrived in valletta, malta where she signed autographs,
appeared on television stations, and gave interviews to the local media.
following malta, she traveled to serbia and montenegro where she gave
additional interviews before moving on to and\\\\ and her low hip@-@
grind during' rude boy' were the smash hits of her body language."
deborah linton of city life wrote that rihanna" even manages to make a
psychiatric couch look sexy". linton called the show' s stage sets
impressive and imaginative. rick massimo of the providence journal wrote
that rihanna" looked like a neon@-@ sign rendition of herself during'
rehab', rarely addressed the audience, and didn' t rise above flat
cliche in that until the very end of the show"." rehab" and rihanna' s
2009 single" russian roulette" were excluded from the set\\\\ only a few
hours. he said:" there were a lot of tracks, but i just enjoyed it, to
be honest. i knew how i wanted it to sound, and it was pretty much the
last song we cut; a lot of the mixing was nailed in the production as
well, which helped. dream did a great job producing this track." the bar
one guitar track of" schoolin' life" was entirely programmed. similarly,
the live drum section in the hook was actually done with programmed
drums. once the mixing was over, swivel' s impression were as
follows:{[}' schoolin' life{]} absolutely\\\\ tour began on march 1,
2000 at the house of blues in los angeles, while other venues included
paris olympia, trump taj mahal, brixton academy, the montreux jazz
festival, and the essence jazz festival in new orleans. by july, the
tour' s first half had sold out in each city. the tour lasted nearly
eight months, whil e performances went for up to three hours a night.
the voodoo tour was taken internationally, with one of the most notable
performances being the free jazz festival in brazil. the music video
for" untitled( how does it feel)" portrayed d' angelo as a sex
symbol\\\\ hobson noted that rihanna" rejects the victim stance" in the
video for" man down", and elucidated that she played the role of a rape
survivor who shot her attacker. she attributed the location of shooting
the video in jamaica as significant, due to how the image of a gun
proliferated during 1990s jamaican dance hall' s to" express female
rage``. the prologue depicts rihanna as a'' dark@-@ hooded" femme fatale
whereby the narrative explains her motives for murder and provokes the
spectator to sympathize with her because she danced in a provocative
manner with a man in a club, which\\\\ had a deep impact on delonge in
that he spent a night up crying for him when he wrote the track." a
little' s enough" was inspired by a religious concept in which a god
came to bring positive change on earth when it faces terrorism, war or
famine." the war", an anthem about the iraq war and its death toll, is
succeeded by" it hurts", a track about a friend of delonge with a
cheating girlfriend." it' s a terrible situation where my friend is
being crushed from the inside out by all the manipulative stuff she' s
doing and this song' s\\\\ just took that dress out of the storage -- it
has a 27@-@ foot train and it was just all hand@-@ beaded and stuff and
so i figured we might as well get a use out of it.'=== synopsis=== the
video features carey readying for her wedding, and follows her to the
altar, as well as her escape from the reception. many of the actors
featured in carey' s" it' s like that" video were in that of" we belong
together", which was shot as a continuation from the" it' s like that"
video. it begins with\\\\ 3 in dutch@-@ speaking flanders and number 2
in french@-@ speaking wallonia. it was certified gold by the belgian
entertainment association( bea) for selling more than 15@,@ 000 copies.
although the song spent only 1 week on the italian singles chart( at
number 8), it was certified platinum by the federazione industria
musicale italiana( fimi) in 2014 for selling more than 30@,@ 000
copies.== music video===== background and synopsis=== anthony mandler
directed the music video for" man down" in april 2011 on a beach in\\\\
at numbers 18 and 43 in the united states, and experienced moderate
success worldwide. unlike her previous records, spears did not heavily
promote blackout; her only televised appearance for blackout was a
universally@-@ panned performance of" gimme more" at the 2007 mtv video
music awards.== background and development== in november 2003, while
promoting her fourth studio album in the zone, spears told entertainment
weekly that she was already writing songs for her next album and was
also hoping to start her own record label in 2004. henrik jonback
confirmed that he had written songs with her during the european leg of
the onyx hotel tour,"\\\\ of albums also had increased sales due to
discounting and publicity generated by the single and her performance.
billboard estimated that her top@-@ 10 digital sales collectively
increased over 1@,@ 700 percent. madonna' s bestselling album was the
2009 greatest@-@ hits collection, celebration, which sold 16@,@ 000
copies( up 1@,@ 341 percent) and reentered the billboard 200 album
chart. the following week celebration fell 105 spots on the chart to
number 157, with sales falling to 4@,@ 000 copies." give me all your
luvin'" fell to number 39 on the hot\\\\ opened the performance with"
yeah 3x" and was dressed in a white formal suit, accompanied by" full@-@
skirted dancers". brown was eventually joined onstage by tuxedo@-@ clad
dancers and began dancing to the 1993 wu@-@ tang clan single" protect ya
neck". his dance routine then moved into 1991, where he danced to
nirvana' s" smells like teen spirit". brown' s performance then came
back to the future, where he began to sing" beautiful people". while
performing the song, he was suspended in the air, and then lowered to
another stage where he continued to\\\\ register that she didn' t know
she had." from the moment she was signed in the film, madonna had
expressed interest in recording a dance version of" don' t cry for me
argentina". according to her publicist liz rosenberg," since she didn' t
write the music and lyrics, she wanted her signature on that
song\ldots{} i think on her mind, the best way to do it was go in the
studio and work up a remix". for this, in august 1996, while still
mixing the film' s soundtrack, madonna hired remixers pablo flores and
javier garza. according to flores, the singer\\\\ d accumulated until
then but that was instead an ideal marriage of production and
performance." instead, the red lights on the stage played up the"
ominous" tone of the song as it gradually increased its tempo to the
point whereby the end of the song was on the verge of sounding like an
incantation. for the diamonds world tour, rihanna performed" man down"
in a caribbean@-@ theme section of the show, which also included" you da
one"," no love allowed``,'' what' s my name?" and" rude boy". james
lachno of the telegraph highlight the caribbean@-@ themed\\\\ edge of
several realities: the film, the dream it inspires, the waking world it
illuminates". the music in" i just can' t stop loving you", a duet with
siedah garrett, consisted mainly of finger snaps and timpani." just good
friends", a duet with stevie wonder, was viewed by critics as sounding
good at the beginning of the song, ending with a" chin@-@ bobbing
cheerfulness``.'' the way you make me feel"' s music consisted of blues
harmonies. the lyrics of" another part of me" deal with being united,
as" we\\\\ not manufactured. no one paid these kids."=== live
performances=== one direction performed" what makes you beautiful" on
red or black? on 10 september 2011. the performance started with hosts
ant\& dec announcing that the band was supposedly running late for their
appearance, and cut to a video of one direction boarding a london tube
carriage full of fans, as the studio version of the song began playing.
each fan on the tube was given a numbered ticket. the band and fans
disembarked the tube and made their way to the television studio, where
the remainder of the song was sung live. after the song,\\\\

